Distribution approximations for the chemical master equation: comparison of the method of moments and the system size expansion

The stochastic nature of chemical reactions involving randomly fluctuating population sizes has lead to a growing research interest in discrete-state stochastic models and their analysis. A widely-used approach is the description of the temporal evolution of the system in terms of a chemical master equation (CME). In this paper we study two approaches for approximating the underlying probability distributions of the CME. The first approach is based on an integration of the statistical moments and the reconstruction of the distribution based on the maximum entropy principle. The second approach relies on an analytical approximation of the probability distribution of the CME using the system size expansion, considering higher-order terms than the linear noise approximation. We consider gene expression networks with unimodal and multimodal protein distributions to compare the accuracy of the two approaches. We find that both methods provide accurate approximations to the distributions of the CME while having different benefits and limitations in applications.

==> discussion.tex <==
% !TEX root =  mcsmain.tex

Final discussion here

 

==> ln.tex <==
% !TEX root =  mcsmain.tex

\subsection{System Size Expansion}
\label{sec:ln}


\subsection{Hybrid System Size Expansion} 
\label{sec:hln}
